Monge blunts Bayes: Hardness Results for Adversarial Training

The last few years have seen a staggering number of empirical studies of the robustness of neural networks in a model of adversarial perturbations of their inputs. Most rely on an adversary which carries out local modifications within prescribed balls. None however has so far questioned the broader picture: how to frame a resource-bounded adversary so that it can be severely detrimental to learning, a non-trivial problem which entails at a minimum the choice of loss and classifiers. We suggest a formal answer for losses that satisfy the minimal statistical requirement of being proper. We pin down a simple sufficient property for any given class of adversaries to be detrimental to learning, involving a central measure of "harmfulness" which generalizes the well-known class of integral probability metrics. A key feature of our result is that it holds for all proper losses, and for a popular subset of these, the optimisation of this central measure appears to be independent of the loss. When classifiers are Lipschitz -- a now popular approach in adversarial training --, this optimisation resorts to optimal transport to make a low-budget compression of class marginals. Toy experiments reveal a finding recently separately observed: training against a sufficiently budgeted adversary of this kind improves generalization.

==> content/impossibility-old.tex <==
% !TEX root=../nips18-adversarial-mf-1.tex

\section{The hardness theorem}\label{sec-imp}

We now show a lower bound on the adversarial loss of \eqref{eqn:adversarial-loss}.
This pins down a
function whose minimisation by the adversary is instrumental to defeat $\mathcal{H}$.

\begin{theorem}\label{thPCL}
For any proper loss $\properloss$, link $\psi$ 
and any $(\mathcal{H}, \mathcal{A})$
integrable with respect to $D$ 
\begin{eqnarray}
\properloss(\mathcal{H}, \mathcal{A},
D) & \geq &\left(\properloss^\circ - \frac{1}{2} \cdot
  \min_{a \in \mathcal{A}} \beta_a \right)_+,
\end{eqnarray}
where $x_+ \defeq \max\{0, x\}$,
and for convenience
\begin{eqnarray}
\beta_a & \defeq & \upgamma^g_{\mathcal{H}, a} (P, N, \pi,
  2\cbr(1), 2\cbr(0)),
\end{eqnarray}
with 
\begin{eqnarray}
g & \defeq & (-\cbr') \circ \psi^{-1}. \label{defgg}
\end{eqnarray}
Hence, if there exists $\epsilon \in [0,1]$
% AKM: edit
% AKM: added here
and $a \in \mathcal{A}$
such that
\begin{eqnarray}
% AKM: edit
%\exists a \in \mathcal{A} : \beta_a  & \leq & 2\epsilon
\beta_a  & \leq & 2\epsilon
\properloss^\circ,\label{bdefeat} 
\end{eqnarray}
then $\mathcal{H}$ is $\epsilon$-defeated by $\mathcal{A}$ on $\properloss$.
\end{theorem}
(Proof in \supplement, Section \ref{proof_thPCL}) We remark that
whenever $\ell$ is canonical, $g = \mathrm{Id}$ and so
\begin{eqnarray}
\beta_a & = & \upgamma_{\mathcal{H}, a} (P, N, \pi,
  2\cbr(1), 2\cbr(0)), 
\end{eqnarray}
so the optimisation of $\upgamma_{\mathcal{H}, a}$ does \textit{not} depend on the loss at
hand --- hence, its optimisation by an adversary could be done without
knowing the loss that the learner is going to minimise. We also remark
that the condition for $\mathcal{H}$ to be $\epsilon$-defeated by
$\mathcal{A}$ does not involve an algorithmic component: it means that
\textit{any} learning algorithm minimising loss $\ell$ will end up
with a poor predictor if \eqref{bdefeat} is satisfied, regardless of
its computational resources.

% AKM: edit
\noindent Broadly, the message is the following:
  \begin{tcolorbox}[colframe=blue,boxrule=0.5pt,arc=4pt,left=6pt,right=6pt,top=6pt,bottom=6pt,boxsep=0pt]
    \begin{center}
      If an adversary drives $\gamma^{[g]}_{\mathcal{H}, a}$ sufficiently small, then every learner minimising a [canonical] proper loss will be defeated.
    \end{center}
  \end{tcolorbox}

% AKM: edit
\noindent Of course, this raises the question of what realistic classes of adversary $\mathcal{A}$ and model $\mathcal{H}$ can be so constructed.
Before detailing this,
we note
several useful corollaries to Theorem \ref{thPCL}.
% There are several
% example of corollaries to Theorem \ref{thPCL} that are worth mentioning.\\

\noindent $\triangleright$ \emph{Relationships with integral probability metrics}.
In a special case, 
the somewhat abstract quantity $\upgamma^g_{\mathcal{H}, a}$ can be related to the more familiar class of integral probability metrics (IPMs)~\citep{sfgslOI}.  
Recall that the latter are a class of metrics on probability distributions,
capturing for example the total variation divergence, Wasserstein distance, and maximum mean discrepancy.

\begin{corollary}\label{corIPM}
Suppose that $\upgammaellpi = 0$ and
$\mathcal{H}$ is closed by negation. Then
\begin{eqnarray}
2 \cdot \upgamma^g_{\mathcal{H}, a} (P, N, \pi,
  2\cbr(1), 2\cbr(0)) & = & \max_{h \in \mathcal{H}} \left|
    \int_{\mathcal{X}} g\circ h\circ a(\ve{x}) \mathrm{d}P(\ve{x})-\int_{\mathcal{X}} g\circ h\circ a(\ve{x}) \mathrm{d}N(\ve{x})\right|,
\end{eqnarray}
which is the integral probability metric for the class $\{g\circ h\circ
a : h \in \mathcal{H}\}$ on $P$ and $N$. Here, $g$ is defined in \eqref{defgg}.
\end{corollary}
The proof is immediate.
% AKM: edit
%Returning to Theorem \ref{thPCL}, we can interpret the result as saying:
We may now interpret Theorem \ref{thPCL} as saying:
for an adversary to defeat a learner minimising a canonical proper loss,
it suffices to make a suitable IPM between the class-conditionals $P, N$ small.
The particular choice of IPM arises from the learner's choice of hypothesis class, $\mathcal{H}$.
Of particular interest is when this comprises kernelised scorers,
as we now detail.


\noindent $\triangleright$ \emph{Relationships with the maximum mean discrepancy}.
The maximum mean discrepancy (MMD)~\citep{gbrssAK} corresponds to an IPM where $\mathcal{H}$ is the unit-ball in an RKHS.
We have the following re-expression of $\gamma_{\mathcal{H}, a}$ for this hypothesis class,
% AKM: edit
which turns out to be a form of weighted MMD.

\begin{corollary}\label{corMMD}
Suppose $\ell$ is canonical proper and let $\mathcal{H}$ denote the unit ball of a
reproducing kernel
Hilbert space (RKHS) of functions with reproducing kernel $\kappa$.
Denote 
\begin{eqnarray}
\mu_{a, Q} & \defeq & \int_{\mathcal{X}} \kappa( a(\ve{x}), .)
    \mathrm{d}Q(\ve{x})
\end{eqnarray}
the adversarial mean embedding of $a$ on $Q$. Then 
\begin{eqnarray*}
2 \cdot \upgamma_{\mathcal{H}, a} (P, N, \pi,
  2\cbr(1), 2\cbr(0)) & = &  \upgammaellpi + \|\pi \cdot \mu_{a, P} - (1-\pi) \cdot \mu_{a, N}\|_{\mathcal{H}}  .
\end{eqnarray*}
\begin{figure}[t]
%\vspace{-20px}
\centering
\includegraphics[trim=20bp 350bp 600bp
30bp,clip,width=.50\linewidth]{Figs/FigLBar} 
\caption{Suppose an adversary $a$ can guarantee an upperbound on
  $\textsc{mmd}_\pi \defeq \|\pi \cdot \mu_{a, P} - (1-\pi) \cdot
  \mu_{a, N}\|_{\mathcal{H}}$ as displayed in thick red. For some
  fixed $\ell / \cbr$ and $\epsilon$, we display the range of $\pi$ values
  (in pink) for which $a$ $\epsilon$-defeats $\mathcal{H}$. Notice
  that outside this interval, it may not be possible for $a$ to
  $\epsilon$-defeat $\mathcal{H}$ (in grey, tagged "?"), and if $\pi$ is large enough
  (orange, tagged "safe"), then it is not possible for condition \eqref{bdefeat} to
  be satisfied anymore (see text for details, best viewed in color).\label{fig:lbar}}
\end{figure}
\end{corollary}
\begin{myproofsketch} It comes from the
reproducing property of $\mathcal{H}$,
\begin{eqnarray}
\lefteqn{2 \cdot \upgamma_{\mathcal{H}, a} (P, N, \pi,
  2\cbr(1), 2\cbr(0))}\nonumber\\
 & = & \upgammaellpi + \max_{h \in \mathcal{H}}
  \left\{\pi \cdot \int_{\mathcal{X}} h\circ a(\ve{x})
    \mathrm{d}P(\ve{x})-(1-\pi) \cdot \int_{\mathcal{X}} h\circ a(\ve{x})
    \mathrm{d}N(\ve{x})\right\}\nonumber\\
 & = &  \upgammaellpi + \max_{h \in \mathcal{H}}
  \left\{\pi \cdot \left\langle h, \int_{\mathcal{X}} \kappa( a(\ve{x}), .)
    \mathrm{d}P(\ve{x})\right\rangle_{\mathcal{H}} -(1-\pi) \cdot \left\langle h, \int_{\mathcal{X}} \kappa( a(\ve{x}), .)
    \mathrm{d}N(\ve{x})\right\rangle_{\mathcal{H}}\right\}\nonumber\\
 & = &  \upgammaellpi + \max_{h \in \mathcal{H}}
  \left\{\left\langle h, \pi \cdot \mu_{a, P} - (1-\pi) \cdot \mu_{a, N}\right\rangle_{\mathcal{H}} \right\}\nonumber\\
 & = &  \upgammaellpi + \|\pi \cdot \mu_{a, P} - (1-\pi) \cdot \mu_{a, N}\|_{\mathcal{H}} ,
\end{eqnarray}
as claimed, where the last equality holds for the unit ball.
\end{myproofsketch}\\
% RN : check that one
%An interesting and more general result holds when relaxing the
%condition on $\ell$ to be canonical: if $g$ in \eqref{defgg} is
%$K$-Lipschitz, then Corollary \ref{corMMD} holds as well for the unit ball
%RKHS defined from $\{g \circ h\}_{h \in \mathcal{H}}$ \cite{XXX}. The Lipschitz
%condition can be found equivalent to have:
%\begin{eqnarray}
%(\cbr)'(y) - (\cbr)'(y') & \leq & K |\Psi(y) - \Psi(y')|, \forall y,
%y' \in [0,1],
%\end{eqnarray}
%which therefore constrains the variations of the canonical link to
%those of the chosen link $\Psi$. 
We finally remark that when $\upgammaellpi = 0$, 
\begin{eqnarray}
2 \cdot \upgamma_{\mathcal{H}, a} (P, N, \pi, 2\cbr(1), 2\cbr(0)) & =
& \|\pi \cdot \mu_{a, P} - (1-\pi) \cdot \mu_{a, N}\|_{\mathcal{H}}, \label{eqMMDpi}
\end{eqnarray}
which is a distance between the weighted mean embeddings of the class-conditionals.
% AKM: edit
This is seen to be a kind of weighted MMD;
if furthermore $\pi = 1/2$ as well,
$$ 2 \cdot \upgamma_{\mathcal{H}, a} (P, N, \pi, 2\cbr(1), 2\cbr(0)) = \frac{1}{2} \cdot \| \mu_{a, P} - \mu_{a, N}\|_{\mathcal{H}},  $$
with the right-hand side exactly being the MMD between $P$ and $N$.
% AKM: edit
This is equally implied by specialising Corollary \ref{corIPM} to this
case.
Figure \ref{fig:lbar} displays an example picture for some canonical
proper but asymetric
loss ($\cbr(0) \neq \cbr(1)$) when an adversary with a given
upperbound guarantee
on the right hand-side of \eqref{eqMMDpi} can indeed $\epsilon$-defeat
some $\mathcal{H}$. We remark that while this may be possible for a whole
range of $\pi$, this may not be possible for all. The picture would be
different if the loss were symmetric (see Corollary \ref{corSYML}
below), since in this case a guarantee to $\epsilon$-defeat
$\mathcal{H}$ for \textit{some} $\pi$ would imply a guarantee for
all. This asymmetry represents
a difficulty for the adversary which, we recall, cannot act on $\pi$.

\noindent $\triangleright$ \emph{Simultaneously defeating
  $\mathcal{H}$ over \textbf{sets} of losses}. While the computation
or the minimization
of $\beta_a$ does not involve the loss used by the learner, satisfying
\eqref{bdefeat} involves the knowledge of one value of this loss, if not
of the loss itself. It turns out that if the adversary has just a
partial knowledge of the loss being optimized in the form of a set of
losses from which the learner picks its loss, it may in fact still be possible
for him to guess whether \eqref{bdefeat} can be satisfied over this
set, as we now show.

\begin{corollary}\label{corSYML}
Let $\mathcal{L}$ be a set of canonical proper losses satisfying the
following property: $\forall \properloss \in \mathcal{L}, \exists
\cbr^\dagger\in \mathbb{R}$ such that $\cbr(1) = \cbr(0)
\defeq \cbr^\dagger$. Assuming $(\mathcal{H}, \mathcal{A})$
integrable with respect to $D$, if 
\begin{eqnarray}
\exists a \in \mathcal{A} : \upgamma_{\mathcal{H}, a} (P, N, \pi,
  0, 0) & \leq & \epsilon  \cdot \inf_{\ell \in
  \mathcal{L}} \properloss^\circ - \cbr^\dagger,
\end{eqnarray}
then $\mathcal{H}$ is simultaneously $\epsilon$-defeated by $\mathcal{A}$ on
\textbf{all} losses of $\mathcal{L}$.
\end{corollary}
The result easily follows from remarking that we have in this case
\begin{eqnarray}
\upgamma_{\mathcal{H}, a} (P, N, \pi,
  2\cbr(1), 2\cbr(0)) & = & 2 \cbr^\dagger + \upgamma_{\mathcal{H}, a} (P, N, \pi,
  0, 0),
\end{eqnarray}
which we then plug in \eqref{bdefeat} to get the statement of the
Corollary. Corollary \ref{corSYML} is interesting for two reasons.
First, it applies to all
proper symmetric losses \citep{nnOT,rwCB}, which includes popular
losses like the square, logistic and Matsushita losses. Finally, it does not
just offer the adversarial strategy to defeat classifiers that would
be learned on any of such losses, it also applies to more
sophisticated learning strategies that would \textit{tune} the loss at
learning time \citep{nnOT,rwCB} or \textit{tailor} the loss to
specific constraints \citep{bssLF}, hence offering a wide attack angle on
training. 

